A Dynamic Cooler Model for Cement Clinker Production

We present a 2D model for a grate belt cooler in the pyro-section of a cement plant. The model is formulated as an index-1 differential-algebraic equation (DAE) model based on first engineering principles. The model systematically integrates thermo-physical aspects, transport phenomena, reaction kinetics, mass and energy balances, and algebraic volume and energy relations. The model is used for dynamic simulation of the cooler and the paper provides dynamic and steady-state simulation results matching the expected behavior. The cooler model is one part of a full pyro-section model for dynamical simulations. The model can serve as a basis for the design of optimization and control systems towards improving energy efficiency and CO2 emission.

==> Nomenclature.tex <==

\printnomenclature

% Notation
\nomenclature{\(Q\)}{heat flow, $J/s$}
\nomenclature[N]{\(H\)}{enthalpy, $J$}
\nomenclature[N]{\(U\)}{internal energy, $J$}
\nomenclature[N]{\(P\)}{pressure, $bar$}
\nomenclature[N]{\(T\)}{temperature, $K$}
\nomenclature[N]{\(C\)}{concentration, $\frac{mol}{m^3}$}
\nomenclature{\(N\)}{material flux, $\frac{mol}{m^2s}$}
\nomenclature[N]{\(V\)}{volume, $m^3$}
\nomenclature{\(v\)}{velocity, $m/s$}
\nomenclature{\(J\)}{Diffusion, $\frac{mol}{m^2s}$}


\nomenclature{\(\hat{X}\)}{density of X, $\frac{[X]}{m^3}$}
\nomenclature{\(\tilde{X}\)}{flux of X, $\frac{[X]}{m^2s}$}
\nomenclature{\(\omega\)}{ rotational velocity, $\frac{r}{s}$}
\nomenclature{\(D_H\)}{ hydraulic diameter, $m$}
\nomenclature{\(D_e\)}{ effective diameter, $m$}

\nomenclature{\(n\)}{ amount of substance, $mol$}

\nomenclature{\(Re\)}{Reynold's number}
\nomenclature{\(E_A\)}{Activation energy, $J/mol$}
\nomenclature{\(x\)}{mole fraction}

\nomenclature{\(S\)}{stoichiometric coefficient matrix}
\nomenclature{\(r\)}{ reaction rate, $\frac{mol}{m^3s}$}
\nomenclature{\(R\)}{ production rate, $\frac{mol}{m^3s}$}
\nomenclature{\(m\)}{ mass, $kg$}
\nomenclature{\(\dot{m}\)}{mass rate, $kg/s$}

% physics
\nomenclature[P]{\( [x]\)}{unit of x}
\nomenclature[P]{\(\sigma\)}{Stefan-Boltzmann's constant, $5.670374419...*10^{-8}Wm^{-2}K^{-4}$}
\nomenclature[P]{\(\mu\)}{viscosity}
\nomenclature[P]{\(\rho\)}{mass density, $\frac{kg}{m^3}$}
\nomenclature[P]{\(M\)}{Molar weight, $\frac{g}{mol}$}
\nomenclature[P]{\(k\)}{conductivity, $\frac{J}{m s K}$}
\nomenclature[P]{\(c_m\)}{ molar thermal capacity}
\nomenclature[P]{\(\epsilon\)}{emissitivity}
\nomenclature[P]{\(\alpha\)}{absorptivity}
\nomenclature[P]{\(\alpha_B\)}{thermal diffusitivity}
\nomenclature[P]{\( V_{\sum} \)}{summed diffusion volume, $m^3$}

% Math
\nomenclature[M]{\(\Delta x\)}{difference of x, $[x]$}
\nomenclature[M]{\(\partial_x\)}{derivative w.r.t. x, $\pdv{}{x}$}

%Geometry
\nomenclature[G]{\(\theta\)}{ fill angle, $rad$}
\nomenclature[G]{\(\phi\)}{slope of bed height w.r.t. kiln axis, $rad$}
\nomenclature[G]{\(\psi\)}{kiln inclination angle}
\nomenclature[G]{\(\xi\)}{angle of bed repose}
\nomenclature[G]{\(A\)}{Area, $m^2$}
\nomenclature[G]{\(h\)}{ bed height,$m$}
\nomenclature[G]{\(V_{\Delta}\)}{ total segment volume,$m^3$}
\nomenclature[G]{\(r_c\)}{ kiln inner cross radius, $m$}
\nomenclature[G]{\(L\)}{ kiln length, $m$}
\nomenclature[G]{\(L_c\)}{ bed surface width, $m$}

 %subscripts / superscript
\nomenclature[S]{\(s\)}{Solid}
\nomenclature[S]{\(g\)}{Gas}
\nomenclature[S]{\(w\)}{Wall}
\nomenclature[S]{\(k\)}{Spatial location}
\nomenclature[S]{\(f\)}{fuel}
\nomenclature[S]{\(air\)}{air intake}
\nomenclature[S]{\(rad\)}{radiation}
\nomenclature[S]{\(cv\)}{convection}


